Optimal Server Selection for Straggler Mitigation

The performance of large-scale distributed compute systems is adversely impacted by stragglers when the execution time of a job is uncertain. To manage stragglers, we consider a multi-fork approach for job scheduling, where additional parallel servers are added at forking instants. In terms of the forking instants and the number of additional servers, we compute the job completion time and the cost of server utilization when the task processing times are assumed to have a shifted exponential distribution. We use this study to provide insights into the scheduling design of the forking instants and the associated number of additional servers to be started. Numerical results demonstrate orders of magnitude improvement in cost in the regime of low completion times as compared to the prior works.

==> Figures/ForkingProcess.tex <==
\pgfplotsset{
every axis/.append style={
axis x line=middle,    % put the x axis in the middle
axis y line=middle,    % put the y axis in the middle
ticks=both,
xtick={0,1,2,4,8},
ytick={1,2,4,7,9,12},
yticklabels={$N_{0}$,$N_{1}$,$N_{2}$,$N_{3}$,$N_4$,$N$},
xticklabels={$t_0$,$t_{1}$,$t_{2}$,$t_{3}$,$$,$$,$t_{m}$} ,
xlabel near ticks,
ylabel near ticks,
xlabel={Forking times},
ylabel={Number of active replicas $N(t)$},
}
}
\begin{tikzpicture}
font=\small,
\begin{axis} [xtick=data,xmin=0,xmax=12, ymin=0, ymax=14, unbounded coords=jump]   
    \addplot[blue, thick, mark=][const plot] coordinates{(0,1) (1,2) (2,4) (4,7) (4.5,7) (7,inf) (8,9.4)(8,10) (10,12) (12,12)};
    \addplot[blue, thick, dashed]coordinates{(4.8,7.2)(7.8,9.2)};
\end{axis}
\end{tikzpicture}



==> Figures/IntroFig.tex <==
\begin{tikzpicture}
  \begin{axis}  
    \addplot+[blue][const plot] coordinates{(0,0) (1.5,2) (2,2.5) (3,3) (4,4)[domain=0:4,blue]};
    \draw[dotted] (axis cs:4.5,3.5) -- (axis cs:7,6.5);
    \addplot+[blue][const plot] coordinates{(7,7) (8,8) (9,9)(10,10)[domain=7:8,blue]};
  \end{axis}
\end{tikzpicture}

